Towards Automated Situation Awareness: A RAG-Based Framework for Peacebuilding Reports

Timely and accurate situation awareness is vital for decision-making in humanitarian response, conflict monitoring, and early warning and early action. However, the manual analysis of vast and heterogeneous data sources often results in delays, limiting the effectiveness of interventions. This paper introduces a dynamic Retrieval-Augmented Generation (RAG) system that autonomously generates situation awareness reports by integrating real-time data from diverse sources, including news articles, conflict event databases, and economic indicators. Our system constructs query-specific knowledge bases on demand, ensuring timely, relevant, and accurate insights. To ensure the quality of generated reports, we propose a three-level evaluation framework that combines semantic similarity metrics, factual consistency checks, and expert feedback. The first level employs automated NLP metrics to assess coherence and factual accuracy. The second level involves human expert evaluation to verify the relevance and completeness of the reports. The third level utilizes LLM-as-a-Judge, where large language models provide an additional layer of assessment to ensure robustness. The system is tested across multiple real-world scenarios, demonstrating its effectiveness in producing coherent, insightful, and actionable reports. By automating report generation, our approach reduces the burden on human analysts and accelerates decision-making processes. To promote reproducibility and further research, we openly share our code and evaluation tools with the community via GitHub.

==> litrev.tex <==
Retrieval-Augmented Generation (RAG) represents an advanced methodology that combines the generative capabilities of large language models (LLMs) with the precision of information retrieval systems. By integrating external knowledge sources, RAG enhances the contextual relevance and factual accuracy of generated content. This hybrid approach has found applications across various domains, including safety, finance, healthcare, and scientific research, offering notable improvements in the quality and efficiency of report generation. The diverse methods of implementing this framework underscore its substantial benefits \cite{gao2023retrieval,fan2024survey,arslan2024survey}. Recently, the RAG architecture has been increasingly adopted across multiple domains.

\textit{RAG in Safety Report Generation.} In the domain of safety, RAG frameworks have been customized to produce comprehensive reports based on work session descriptions and logs. These systems leverage models such as LLaMA and employ various embedding techniques to automate the generation of safety reports that comply with stringent documentation standards. Studies utilizing aviation safety datasets have demonstrated the effectiveness of RAG models in improving report accuracy and efficiency, with performance metrics such as Recall@5, GLEU, METEOR, and BERTScore showcasing significant enhancements over traditional reporting methods \cite{Bernardi2024Automatic}. 

\textit{RAG for Financial Report Analysis.} The financial sector has adopted RAG to enhance the analysis and interpretation of financial reports, particularly in question-answering tasks for private investors \cite{Iaroshev2024Evaluating}. Models like OpenAI's ADA and GPT-4 have been employed to process half-yearly and quarterly reports with high accuracy and contextual relevance. Research findings indicate that the quality of financial report structuring plays a crucial role in optimizing RAG performance, especially when addressing qualitative queries.

\textit{RAG in Medical Report Writing.} Healthcare applications of RAG, particularly in radiology, involve the automated generation of radiology reports through the use of multimodal embeddings \cite{Ranjit2023Retrieval}. These embeddings facilitate the retrieval of relevant radiology texts, which are then processed by generative models such as OpenAI's GPT series. The integration of user intents and specific clinical requirements into the generative process has resulted in improved clinical metrics, including BERTScore and Semb score, while also mitigating issues related to hallucinated content. This and other application of RAG framework for report automation in medicine are showing promising results \cite{markey2024rags,Wang2024Optimizing,Assistant2024A,alam2024towards}


\textit{Scientific Research Summarization Using RAG.} In the context of large-scale scientific research, RAG-based summarization agents have been deployed to manage and synthesize vast volumes of information \cite{Suresh2024Towards}. These agents utilize vector databases to retrieve relevant content, enabling LLMs to generate concise summaries enriched with citations. The application of RAG in scientific research not only enhances data comprehension but also fosters collaborative engagement among researchers.

\textit{RAG and Broader NLP Applications in Peacebuilding.} While advancements in Natural Language Processing (NLP), particularly the integration of Large Language Models (LLMs) with Retrieval-Augmented Generation (RAG), have demonstrated significant benefits across various domains, their application in peacebuilding remains an emerging area of exploration. Although progress has been made, the adoption of these technologies for conflict prevention, resolution, and post-conflict recovery is still in its early stages. Nevertheless, recent research has successfully leveraged advanced NLP techniques for conflict prediction and the monitoring of human rights violations \cite{Trivedi2020How,Alhelbawy2020An,Mueller2024Introducing,Nemkova2023Detecting}. These developments highlight the potential for further integration of RAG and other NLP methodologies to support peacebuilding initiatives and humanitarian efforts.

\textit{Multimodal RAG Systems.} The development of multimodal RAG systems has expanded the capabilities of report generation by incorporating diverse data types, including text, tables, and images. These systems improve retrieval and content generation by considering interrelationships between different modalities. Empirical evaluations across multiple datasets have demonstrated the effectiveness of multimodal RAG in generating accurate and contextually enriched reports\cite{Joshi2024Robust,Xia2024MMed-RAG}. 

\textit{Challenges and Practical Solutions in RAG Implementation. }Despite the promising advancements, the implementation of RAG systems presents several technical challenges, including data preprocessing, retrieval indexing, and response generation. \cite{Khan2024Developing} Practical experience suggests that the integration of generative AI with precise retrieval mechanisms is essential for ensuring transparency, accuracy, and contextual relevance. Solutions such as leveraging OpenAI's Assistant API and LLaMA's open-source models have been proposed to enhance the reliability and robustness of RAG-based applications.


RAG frameworks have demonstrated substantial potential in automating and refining report generation across diverse domains. By integrating retrieval and generation processes, RAG systems provide improved accuracy, contextual relevance, and operational efficiency, making them indispensable tools for professionals in safety, finance, healthcare, and scientific research. The continuous evolution and optimization of RAG technologies promise further advancements in their applicability and effectiveness in various settings.
